Exploration of Time Reversal for Wireless Communications within Computing Packages

Wireless Network-on-Chip (WNoC) is a promising paradigm to overcome the versatility and scalability issues of conventional on-chip networks for current processor chips. However, the chip environment suffers from delay spread which leads to intense Inter-Symbol Interference (ISI). This degrades the signal when transmitting and makes it difficult to achieve the desired Bit Error Rate (BER) in this constraint-driven scenario. Time reversal (TR) is a technique that uses the multipath richness of the channel to overcome the undesired effects of the delay spread. As the flip-chip channel is static and can be characterized beforehand, in this paper we propose to apply TR to the wireless in-package channel. We evaluate the effects of this technique in time and space from an electromagnetic point of view. Furthermore, we study the effectiveness of TR in modulated data communications in terms of BER as a function of transmission rate and power. Our results show not only the spatiotemporal focusing effect of TR in a chip that could lead to multiple spatial channels, but also that transmissions using TR outperform, BER-wise, non-TR transmissions it by an order of magnitude

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/phases.tex <==
\begin{table}
 \caption{Phase distributions leading to the field distribution of \figref{v_h_beams}.}
 \label{table_vertical}
 \begin{tabular}
% %\caption{Phases to create vertical beam}
{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{9}{|c|}{Vertical Beam} \\ \hline
Port & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\ 
Phase & 90 & 120 & 150 & 180 & 0 & 30 & 60 & 90 \\ \hline
Port & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ 
Phase & -90 & -60 & -30 & 0 & -180 & -150 & -120 & -90 \\ \hline
\hline
\multicolumn{9}{|c|}{Horizontal Beam} \\ \hline
Port & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\ 
Phase & 0 & -330 & -300 & -270 & -150 & -120 & -90 & -60 \\ \hline
Port & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ 
Phase & 60 & 90 & 120 & 150 & 270 & 300 & 330 & 0 \\ \hline
\end{tabular}
\end{table}

% \begin{table}
% \caption{Phase distributions leading to the field distribution of \figref{v_h_beams}.}
% \begin{tabular}
% %\caption{Phases to create vertical beam}
% {|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
%  \hline
%  \multicolumn{4}{|c|}{Vertical Beam} \\
%  \hline
%  Port 1 & Port 2 & Port 3 & Port 4\\
%  \hline
%  90   & 120 & 150 &  180\\
%  \hline
%  \hline
%  Port 5 & Port 6 & Port 7 & Port 8\\
%  \hline
%  0   & 30 & 60 &  90\\
%  \hline
%  \hline
%  Port 9 & Port 10 & Port 11 & Port 12\\
%  \hline
%  -90   & -60 &-30 &  0\\
%  \hline
%  \hline
%  Port 13 & Port 14 & Port 15 & Port 16\\
%  \hline
%  -180   & -150 & -120 & -90\\
%  \hline
%  %\caption{Phases to create vertical beam}
% \end{tabular}
% \label{table_vertical}
% \begin{tabular}{ |p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
%  \hline
%  \multicolumn{4}{|c|}{Horizontal Beam} \\
%  \hline
%  Port 1 & Port 2 & Port 3 & Port 4\\
%  \hline
%  0   & -330 & -300 &  -270\\
% \hline
%  \hline
%  Port 5 & Port 6 & Port 7 & Port 8\\
%  \hline
%  -150   & -120 & -90 &  -60\\
%  \hline
%  \hline
%  Port 9 & Port 10 & Port 11 & Port 12\\
%  \hline
%  60   & 90 & 120 &  150\\
%  \hline
%  \hline
%  Port 13 & Port 14 & Port 15 & Port 16\\
%  \hline
%  270   & 300 & 330 & 0\\
%  \hline
% \end{tabular}
% \end{table}
